Substance or Style: What Does Your Image Embedding Know?

Probes are small networks that predict properties of underlying data from embeddings, and they provide a targeted, effective way to illuminate the information contained in embeddings. While analysis through the use of probes has become standard in NLP, there has been much less exploration in vision. Image foundation models have primarily been evaluated for semantic content. Better understanding the non-semantic information in popular embeddings (e.g., MAE, SimCLR, or CLIP) will shed new light both on the training algorithms and on the uses for these foundation models. We design a systematic transformation prediction task and measure the visual content of embeddings along many axes, including image style, quality, and a range of natural and artificial transformations. Surprisingly, six embeddings (including SimCLR) encode enough non-semantic information to identify dozens of transformations. We also consider a generalization task, where we group similar transformations and hold out several for testing. We find that image-text models (CLIP and ALIGN) are better at recognizing new examples of style transfer than masking-based models (CAN and MAE). Overall, our results suggest that the choice of pre-training algorithm impacts the types of information in the embedding, and certain models are better than others for non-semantic downstream tasks.

==> content.tex <==
\begin{abstract}
Foundation models provide a general embedding that can be used for downstream tasks. However, it is unclear what information is kept or lost when going from raw data to a compressed representation. For example, if we blur or add noise to an image, then can we detect this from an embedding like MAE or SimCLR without access to the pixels? To address this, we design a systematic transformation prediction task as a way to probe several popular embeddings. Our task effectively measures the invariance of embeddings. We find that many embeddings do contain enough information to predict image transformations. The subtlety is that post-processing the embedding often improves transformation prediction (e.g., one hidden layer on top of a frozen embedding model). Hence, low-level information may be present but not readily available. We then experiment with various post-processing methods, as a way to fine-tune embeddings to better capture transformation information in addition to semantic content.
\end{abstract}

\section{Introduction}

\label{intro}



Machine learning systems have been making increased use of embedding models as a way to standardize and improve data representations. In particular, the term \emph{foundation model} has been used to describe a `general-purpose’ embedding method~\cite{bommasani2021opportunities}. Training such models typically requires careful tuning and costly compute resources. Fortunately, once they have been trained, these networks can be frozen and made broadly available as an embedding method. While this has many advantages, it also introduces biases depending on what information is kept or lost when moving from raw data to a low-dimensional representation.

Popular vision foundation models learn from large amounts of unlabeled data via self-supervised techniques. For example, contrastive losses like SimCLR~\cite{chen2020simple}, have played an important role in designing image embeddings. During training, the network sees pairs of transformed versions of the same image, and the representation is penalized if the embeddings differ. Intuitively, this suggests that the embedding should be invariant with respect to these transformations, which include cropping, color distortion, and Gaussian blur. Another self-supervised learning method is the Masked AutoEncoder (MAE)~\cite{he2022masked}. The network sees images that have been subject to patch-wise masking, and the goal is to reconstruct the mixing pixels. Since the MAE model has to fill in parts of the image, it is possible that MAE-based embeddings are more aware of visual distortions and stylization.



Evaluation metrics for pre-trained embeddings often focus on semantic accuracy (e.g., ImageNet performance). Moreover, research papers primarily compute metrics by using a linear probe trained on top of a frozen embedding model (possibly after fine-tuning on the target dataset). This is a natural first step because we want embeddings to be immediately useful for downstream tasks, without needing to train large networks on top of the embedding. However, it is not clear what aspects of the embedding contribute to the improved performance of modern embeddings (MAE, SimCLR, CLIP, etc) over traditional supervised methods. A reasonable hypothesis may be that better embeddings have a higher capacity in the sense that they are able to capture more information about the original image. In other words, they are closer to a lossless embedding, which may be desirable if the aim is to have a representation that can be used for many tasks.



\subsection{Predicting Transformations}



One way to scrutinize image embeddings is to modify an image and then see if this change is detectable after computing the image’s embedding. For example, consider two images: one that is a sample from ImageNet, and another where the same image is subject to a small amount of Gaussian blurring. Then, consider computing embeddings for both images, and throwing out the original pixels. Assume that in both cases a linear probe will predict the correct ImageNet class for the image. The next question is: does the embedding contain enough information to determine which image was blurred and which was unaltered? 



If the embedding contains sufficient information to detect blurring, then it should be possible to train a network to perform well on a `blurry or not’ classification task. Specifically, we can apply Gaussian blur to ImageNet, and we can train a network to predict whether the transformation has been applied given access only to the image embeddings. Foundation models that capture more of the transformation information will perform better on this task, whereas models that perform poorly must be insensitive to the transformation. This type of evaluation metric is orthogonal to, and hence complements, existing semantic accuracy measurements for image embeddings.



The usefulness of being sensitive to blurring or other transformations depends on the downstream task. Some embeddings might completely ignore the blurring (leading to a blurring-invariant model) or encode the blurring in a consistent way (leading to a blurring-equivariant model). The former approach has advantages when considering robustness. On the other hand, the latter equivariant approach may be more desirable for data cleaning or content filtering applications, and in general, retaining information about the blurriness would be closer to a lossless representation.



\subsection{Our Contributions}



At a high-level, our aim is to measure the invariance/equivariance of image embeddings. To do so, we propose a new, systematic transformation prediction task. Given a frozen image embedding model and an unseen image, the goal of this task is to predict how the image has been modified (e.g., blurred, noised, stylized, etc). Performance on this task is a way to probe image embeddings and elicit whether or not they capture various changes to an image.



One of our findings is that MAE is more sensitive to transformations than SimCLR. While this may be expected, we also dig into the confusion matrix of the transformation predictions and uncover some insights into the invariances of SimCLR. We also compare to a supervised method and to CLIP and we find TODO….



Another axis is the width of the network that processes the embedding, We experiment with widths as small as XX, and find that the transformation prediction is maintained or only slightly degrades. In other words, the internal layer of small width provides a representation that encodes the transformation with few features.



We then investigate the interplay between semantic prediction (i.e., ImageNet classification) and transformation prediction. For example, we consider whether it is possible to produce a small embedding (64 or 128 dimensions) that performs well on both tasks. TODO… post-processing…



Overall, our analysis sheds new light on image foundation models and offers a simple approach to alter the information in an embedding. We posit that general embeddings should contain both high-level details (semantic class) and low-level modifications (presence of a transformation).



\section{Related Work}

\label{relatedwork}



\textbf{Foundation Models.} Many ML pipelines use image embeddings from pre-trained models instead of training networks on raw image pixels. This is a part of a larger trend of creating and using foundation models, which are very large networks that learn from easy-to-collect data without much supervision~\cite{bommasani2021opportunities}. For vision tasks, SimCLR~\cite{chen2020simple} and MAE~\cite{he2022masked} have recently showcased the impressive capability of learning good image representations in a self-supervised manner. Similar trends appear for language (e.g, BERT~\cite{devlin2018bert} and GPT-3~\cite{brown2020language}), audio (e.g., wav2vec~\cite{Schneider2019}) and multi-modal data (e.g., CLIP~\cite{radford2021learning} and ALIGN~\cite{jia2021scaling}). The good performance and widespread use of foundation models motivates a deeper understanding of what is captured or lost in the embedding process.



\textbf{Invariance and Equivariance.} The popularity of SimCLR has led researchers to question whether embeddings should be encouraged to be insensitive (a.k.a., invariant) or sensitive (a.k.a., equivariant) to transformations~\cite{dangovski2021equivariant, tian2020makes, xiao2021should}. This extends research that aims to better understand rotation prediction~\cite{metzger2020evaluating}, which was a seminal task for unsupervised image representation learning~\cite{komodakis2018unsupervised}. There have also been attempts at using augmentation aware self-supervised learning to improve downstream semantic prediction~\cite{metzger2020evaluating}.



\textbf{Transformation prediction.} Work on visual chirality shows that, surprisingly, it is possible to train a model to detect whether an image has been mirrored~\cite{lin2020visual}. Researchers have identified nuisance factors of X-ray images~\cite{sun2022beyond} even when using a pre-trained chest radiography model~\cite{sellergren2022simplified}. Part of training diffusion models involves reversing the (artificial) Gaussian noise in an image, and part of the optimization involves a noise-prediction loss~\cite{ho2021classifier, ramesh2022hierarchical, song2019generative, yang2022diffusion}. Recent work on cold diffusion considers reversing other transformations, including deblurring, inpainting, super-resolution, and snow removal~\cite{bansal2022cold}. Compared to prior work, our focus is on using transformation prediction as way to probe image embeddings, and we consider a broader set of transformations (e.g., overlays, style transfer, dithering) as well as more variation within similar categories (e.g., hue, saturation, brightness, motion blur).





\section{Probing Embeddings by Predicting Transformations}

\label{probing}



Evaluating only the typical semantic accuracy on class labels leaves open questions regarding what information from the raw data is kept or lost in the embedding. Therefore, we also measure the ability of a network to predict the type of transformation that has been applied to an image. To do so, we define a transformation prediction task along with new metrics. This task can be formulated for any dataset/task as long as there is a way to synthetically apply transformations to all train/test examples.



\subsection{Transformation Prediction Task}



Assume we have T different image transformations. Here, for \emph{transformation}, we take a broad definition. One option is a well-defined function, such as adding Gaussian noise with certain mean/variance independently to each pixel. Another possibility is to have some random parameters, such as choosing a value in a range and increase the image’s saturation by this much. Finally, we can think of transformation families, containing several \emph{sub-transformations}. For example, the family `filtering’ could mean choosing a sub-transformation that modifies hue, brightness, or saturation, and these sub-transformations have their own (possibly random) parameters.



We can apply each of the $T$ transformations to all images in the training and test sets. Including the original images, we will generate $T+1$ copies of the dataset. Similarly, this process defines a $(T+1)$-way classification problem, labeling each image either with `identity’ or one of the $T$ transformations.



\subsection{Metrics} 



We define several metrics based on the fact that we have both unaltered (clean) images and transformed ones, as well as a new `label’ for the type of transformation. For a labeled dataset such as ImageNet, which contains images $x$ and semantic class labels $y$, we will use $t$ to denote the transformation label of our augmented dataset, leading to a labeled triple $(x,y,t)$. A network can predict the semantic label $y$, the transformation label $t$, or both at the same time in a multi-task scenario. 



We measure the \emph{transformation prediction accuracy} as the fraction of images receiving the correct transformation label (the network does not see the class label). We use \emph{clean semantic accuracy} to refer to the fraction of correctly predicted class labels on unaltered images (i.e., the transformation $t$ is the identity). Finally, the \emph{obfuscated semantic accuracy} is the fraction of correct class labels when the image has been transformation in some way (i.e., the transformation $t$ is \emph{not} the identity).



\subsection{Evaluating Image Embeddings}



Consider an image $x$ that has been subject to one of the $T+1$ transformations. For a frozen embedding model $\phi$, the input for our problem will be $\phi(x)$, and we will not have access to $x$ itself. We then train a network that takes $\phi(x)$ as input and outputs a semantic label or a transformation label or both. In a multi-task setting with a two-headed network that outputs two labels, we independently measure the clean/obfuscated semantic and transformation accuracies.



Training a linear probe on top of the embedding $\phi$ is the simplest setting to predict transformation labels. The last-layer weights can be trained using the transformation labels (while the embedding model is fixed). We also consider other post-processing methods. For example, we can use a single hidden layer with varying width instead of a linear probe. In this case, training the hidden layer leads to a new representation that has been fine-tuned for transformation prediction. We can also do this fine-tuning in a multi-task way, incorporating the loss from both the semantic and transformation prediction tasks. 



\subsection{Fine-grained vs.~coarse-grained}



In our experiments, we will consider a fine-grained task (only the parameters vary) and a coarse-grained version (where the same label contains different functions). The latter option allows us to measure generalization accuracy on a hold-out set of sub-transformation. In other words, we can maintain the same label space, and the network can predict on images that have been modified in an unseen way. For all coarse-grained transformations, the test sub-transformations form a superset of the train ones.



The benefit of the fine-grained task is that we can more directly investigate the information in an embedding. We train a small network or a linear probe on top of an embedding. The post-processing network can learn which features of the embedding should correspond to different transformation labels. During test-time, the same transformation applied to an image will only differ in its parameters but not the overall way the image is altered.



The coarse-grained task, on the other hand, allows us to measure a type of generalization. Here the network does not see certain sub-transformations during training. However, we choose the coarse categories so that the visual differences should be similar in some way. For example, the style transfer transformation uses XX styles for the training set and YY for the test set. To correctly label an image, the post-processing network must extract more general information about what style transfer means, instead of relying on a simpler signal such as pixel colors. Hence, the image embedding model needs to retain richer information about the transformation. This leads to the possibility of an embedding being sensitive enough to classify the training sub-transformations, but being too invariant to generalize to unseen sub-transformations.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Post-Processing Embeddings}
\label{postprocessing}

\section{Experimental Results}
\label{experiments}

\textbf{Datasets.} We evaluate on transformed versions of ImageNet~\cite{russakovsky_2015_imagenet}. In addition to the original image (Identity), we apply 30 transformations to each train/test image. This leads 31 classes for the fine-grained transformation prediction task. We also construct a coarse-grained dataset with XXX categories, where each category contains one or more transformations along with a range of parameters (e.g., noise level or type of style transfer). The test set transformations form a superset of those applied to the training images. Full details in \cref{dataset-details}. 

\textbf{Metrics}. We measure the \textit{transformation prediction accuracy} as a multi-class classification problem. In the fine-grained case, the model predicts one of 31 classes. In the coarse-grained case, the model predicts one of XXX classes, which enables us to measure accuracy on unseen transformations. For both cases, we average over a test set with size being the number of original images times the number of labels. We also measure \textit{semantic prediction accuracy} as usual by using the ImageNet class labels.

\textbf{Models}. CAN, MAE, SimCLR, Supervised. All ViT L/16 models pre-trained on JFT. We have used networks with two to eight hidden layers; in some cases, deeper networks achieve higher accuracy, but the difference is small, and the trends remain the same.

\textbf{Research Questions.} We aim to determine: (1) How much transformation information is contained in different embeddings? (2) Can we post-process embeddings to achieve high transformation and semantic accuracies simultaneously? (3) How do other variants, such as dimensionality and training method, affect the transformation accuracy?

\subsection{Results}

\begin{table}[t]
\caption{Transformation prediction accuracies for fine/coarse-grained datasets and various embeddings.}
\label{table:tranformations}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcc}
\toprule
Embedding & Fine-Grained & Coarse-Grained \\
\midrule
CAN & \textbf{98.53} & \textbf{87.72} \\
MAE & 97.65 & 86.83 \\
SimCLR & 93.59 & 87.39 \\
CLIP & x & x \\
Supervised & x & x \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

\begin{table}[t]
\caption{SimCLR transformation prediction accuracies comparing embedding vs.~projection. Networks either have one hidden layer (width $\in\{128, 16k\}$) or just a linear probe.}
\label{table:simclr}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{llcc}
\toprule
Embedding & Dim & Fine & Coarse \\
\midrule
SimCLR embed & 1k $\rightarrow$ 16k & \textbf{93.78} & 86.56 \\
SimCLR embed & 1k $\rightarrow$ 128 & 92.04 & \textbf{87.52} \\
SimCLR embed & lin prob & 89.20 & 87.06\\
SimCLR proj & 128 $\rightarrow$ 16k & 81.50 & 82.15 \\
SimCLR proj & 128 $\rightarrow$ 128 & 74.63 & 80.59 \\
SimCLR proj & lin prob & 71.66 & 76.99 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

\subsection{Discussion}

\subsection{Limitations}

One deficiency of our work is that we have not proposed ways to translate our observations into improvements for benchmark tasks. For example, it would ideal to couple transformation prediction with a new architecture or training algorithm and create a self-supervised learning method that outperforms CAN, MAE, and SimCLR. A different thread could have been using transformation prediction for a data cleaning or filtering task, such as finding anomalous images in a large, but not curated, dataset.Another shortcoming is that our experiments have focused only on image embeddings, but there are also foundation models for text, audio, and other modalities. The transformation prediction task can easily be defined more generally (e.g., for text, we can perturb words via typos or sentences via synonym replacement). Hence, we could have painted a more complete picture by finding themes across embeddings for different modalities. 
\section{Conclusion}
\label{conclusion}

We constructed and investigated a new classification task that allowed us to evaluate the sensitivity of multiple image embeddings to many categories of transformations. Our experiments uncovered some ways in which SimCLR is more invariant than MAE, and the types of transformations that are captured by self-supervised methods but ignored by supervised training. We also demonstrated that it is possible to post-process embeddings using a small network and extract more transformation information compared to using a linear probe. The findings from the transformation prediction task provide new insights into the capacity of image embedding methods, which complements prior experiments on semantic accuracy.

\textbf{Future Work.} Looking forward, a main open question is to create a nearly lossless image embedding that is also easily adapted for many downstream tasks. Our work suggests that it should be possible to keep more low-level information in the representation without compromising semantic performance. Beyond transformations, it would be interesting to encourage embeddings to retain other aspects of an image, such as texture, perspective, or stylistic themes. Another future direction is extending the transformation prediction task to be more fine-grained. For example, we could ask the network to predict the specific parameters or strength of one or more transformations, or to identify which part of an image has been altered. This could uncover further differences between embedding methods.

\bibliography{references}
\bibliographystyle{icml2022}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% APPENDIX
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage
\appendix
\onecolumn

% \section{Further Related Work}

% \section{Other Stuff}

\section{Experimental Set-Up}

\section{Dataset and Transformation Details}
\label{dataset-details}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
